Nonlinear MCMC for Bayesian Machine Learning

We explore the application of a nonlinear MCMC technique first introduced in [1] to problems in Bayesian machine learning. We provide a convergence guarantee in total variation that uses novel results for long-time convergence and large-particle ("propagation of chaos") convergence. We apply this nonlinear MCMC technique to sampling problems including a Bayesian neural network on CIFAR10.

==> neurips7 - camera arxiv/preamble.tex <==
% \usepackage{{../james_package_arxiv}}
\usepackage{{james_package_arxiv}}
\usepackage{mathrsfs}
\usepackage{xcolor}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage[nottoc]{tocbibind}
\usepackage{natbib}
\usepackage{footnotebackref}
\usepackage{multirow}

\usepackage{thmtools,thm-restate}

\usepackage[totoc]{idxlayout}


\newcommand{\calF}{\mathcal{F}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calZ}{\mathcal{Z}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calX}{\mathcal{X}}

\newcommand{\eps}{\epsilon}

\renewcommand{\tr}{\mathrm{tr}}
\newcommand{\eqd}{\overset{d}{=}}
\newcommand{\eqover}[1]{\overset{#1}{=}}
\newcommand{\erf}{\mathrm{erf}}
\renewcommand{\supp}{\mathrm{supp}}
\newcommand{\iid}{\overset{iid}{\sim}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\ent}{\mathrm{Ent}}
% \newcommand{\law}{\mathrm{Law}}
\newcommand{\law}{\mathrm{Distribution}}
\newcommand{\osc}{\mathrm{osc}}

\renewcommand{\P}{\mathds{P}}
\newcommand{\E}{\mathds{E}}
\renewcommand{\Q}{\mathds{Q}}
\newcommand{\K}{\mathds{K}}
\newcommand{\N}{\mathds{N}}
\newcommand{\W}{\mathds{W}}
\renewcommand{\M}{\mathds{M}}
\newcommand{\KL}{\mathds{KL}}
\newcommand{\J}{\mathds{J}}

\newcommand{\scrL}{\mathscr{L}}
\newcommand{\scrV}{\mathscr{V}}
\newcommand{\scrH}{\mathscr{H}}
\newcommand{\scrC}{\mathscr{C}}
\newcommand{\scrB}{\mathscr{B}}

\newcommand{\remph}[1]{{\color{red}#1}}
\newcommand{\gremph}[1]{{\color{gray}#1}}

\newcommand{\james}[1]{{\color{red} #1}}
% \newcommand{\anonymize}[1]{\textless\emph{REDACTED FOR ANONYMITY}\textgreater}
\newcommand{\anonymize}[1]{#1}

\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}

\theoremstyle{plain}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}

% \newcommand{\nnewline}{\newline}
\newcommand{\nnewline}{}

%%% Coloring the comment as blue
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output

\hypersetup{
    colorlinks = true,
    % colorlinks = false,
    linkbordercolor = {white},
    % citecolor = {green},
    citecolor = {red},
    linkcolor = {blue}
}

\renewcommand{\bibname}{References}
% \setlength{\bibsep}{0pt plus 0.3ex}
% \setlength{\bibsep}{0pt plus 0.9ex}
\setlength{\bibsep}{1pt plus 0.3ex}

